Overview of the CLEF-2019 CheckThat!: Automatic Identification and Verification of Claims

We present an overview of the second edition of the CheckThat! Lab at CLEF 2019. The lab featured two tasks in two different languages: English and Arabic. Task 1 (English) challenged the participating systems to predict which claims in a political debate or speech should be prioritized for fact-checking. Task 2 (Arabic) asked to (A) rank a given set of Web pages with respect to a check-worthy claim based on their usefulness for fact-checking that claim, (B) classify these same Web pages according to their degree of usefulness for fact-checking the target claim, (C) identify useful passages from these pages, and (D) use the useful pages to predict the claim's factuality. CheckThat! provided a full evaluation framework, consisting of data in English (derived from fact-checking sources) and Arabic (gathered and annotated from scratch) and evaluation based on mean average precision (MAP) and normalized discounted cumulative gain (nDCG) for ranking, and F1 for classification. A total of 47 teams registered to participate in this lab, and fourteen of them actually submitted runs (compared to nine last year). The evaluation results show that the most successful approaches to Task 1 used various neural networks and logistic regression. As for Task 2, learning-to-rank was used by the highest scoring runs for subtask A, while different classifiers were used in the other subtasks. We release to the research community all datasets from the lab as well as the evaluation scripts, which should enable further research in the important tasks of check-worthiness estimation and automatic claim verification.

==> 2.relwork.tex <==
\section{Related Work}
\label{sec:related}

Journalists, online users, and researchers are well aware of the proliferation of false information, and topics such as credibility and fact-checking are becoming increasingly important. 
For example, there was a 2016 special issue of the ACM Transactions on Information Systems journal on Trust and Veracity of Information in Social Media \cite{Papadopoulos:2016:OSI}, and
there is a Workshop on Fact Extraction and Verification at EMNLP'2018.
Moreover, there is
%have been several related shared tasks, e.g., 
a SemEval-2017 shared task on Rumor Detection \cite{derczynski-EtAl:2017:SemEval}, 
an ongoing FEVER challenge on Fact Extraction and VERification at EMNLP'2018, 
\hl{the current and the previous editions of CheckThat!}\cite{nakov2018overview},
and an upcoming task at SemEval'2019 on Fact-Checking in Community Question Answering Forums.

\noindent Automatic fact-checking was envisioned in \cite{vlachos2014fact} as a multi-step process that includes
(\emph{i})~identifying check-worthy statements 
%from two websites (Channel 4 and politifact.com) 
\cite{gencheva-EtAl:2017:RANLP,hassan2015detecting,NAACL2018:claimrank},
(\emph{ii})~generating questions to be asked about these statements~\cite{karadzhov2017fully},
(\emph{iii})~
retrieving relevant information to create a knowledge base~\cite{shiralkar2017finding}, 
and
(\emph{iv})~inferring the veracity of the statements, e.g., using text analysis~\cite{Castillo:2011:ICT:1963405.1963500,rashkin2017truth}
or external sources~\cite{karadzhov2017fully,Popat:2017:TLE:3041021.3055133}. 

\subsection{Task 1: }
...

\subsection{Task 2: }
...

==> 3.datasets.tex <==
\section{Datasets}
\label{sec:datasets}

We produced the \hl{***} corpus, which stands for CheckThat! 2019 corpus. It is composed of \hl{***} (check-worthiness corpus) and \hl{***} (fact-checking corpus). 

Table~\ref{tab:datasets-overview} gives an overview. 

The training sets for both tasks come from the first and the second Presidential debates and the Vice-Presidential debate in the 2016 US campaign. The labels for both tasks were derived from manual fact-checking analysis published on factcheck.org. For Task 1, a claim was considered check-worthy if a journalist had fact-checked it. For Task 2 a judgment was generated based on the free-text discussion by the fact-checking journalists: true, half-true, or false. 
We followed the same procedure for texts in the test set: two other debates and five speeches by Donald Trump, which occurred after he took office as a US President.
Note that there are cases in which the number of claims intended for predicting factuallity is lower than the reported number of check-worthy claims. The reason is that claims exist which were formulated more than once in both debates and speeches and, whereas we do consider them all as positive instances for Task 1, we consider them only once for Task 2.

\begin{table}[t]
\centering
\begin{tabular}{c @{\hspace{3mm}} l@{\hspace{3mm}}l@{\hspace{3mm}}c @{\hspace{3mm}}c @{\hspace{3mm}}c @{\hspace{3mm}}c @{\hspace{3mm}}c}
\toprule 
 &		 		& \bf Set 	& \bf Claims	& \bf Check-	& \multicolumn{3}{c}{\bf Factuallity}	\\ 
 &		 		& 	 	& 		& \bf worthy	& \bf true	& \bf half-true	& \bf false	\\
 \midrule 
 &  \bf Debates				\\
\faLanguage & 1st Presidential	& training	& 1,403		& 37	& 8	& 9	& 13	\\
\faLanguage & 2nd Presidential	& training	& 1,303		& 25	& 4	& 7	& 14 \\
\faLanguage & Vice-Presidential	& training	& 1,358 	& 28	& 7	& 6	& 14 \\
\faLanguage & 3rd Presidential	& test		& 1,351		& 77	& 19	& 8	& 21 \\
\faLanguage & 9th Democratic	& test		& 1,464 	& 17	& 3	& 3	& 4	\\
  &  \bf D. Trump Speeches	\\
\faLanguage & Acceptance	& test		& \,\,\,375	& 21	& 8	& 5	& 7 \\
  & World Economic Forum 	& test		& \,\,\,245	& 11	& 6	& 2	& 3 \\
  & Tax Reform Event 		& test		& \,\,\,412	& 16	& 4	& 4	& 4 \\
  & Address to Congress		& test		& \,\,\,390	& 15	& 6	& 3	& 4 \\
  & Miami Speech		& test		& \,\,\,645	& 35	& 4	& 9	& 12 \\	
\faCircle &  \bf Snopes.com claims& test	& --		& 150	& 30	& 10	& 110	\\
\bottomrule
\end{tabular}
\caption{\label{tab:datasets-overview}Overview of the debates, speeches, and isolated claims in the \corpus corpus. It includes the number of utterances, those identified as check-worthy (task 1), and those claims identified as factually- true, half-true, and false. The debates/speeches that are available in Arabic are marked with \faLanguage. Note that the claims from snopes.com were released in Arabic only, and are marked with \faCircle.}
\end{table}


